The Power of Interpolation: Understanding the Effectiveness of SGD in Modern Over-parametrized Learning

In this paper we aim to formally explain the phenomenon of fast convergence of SGD observed in modern machine learning. The key observation is that most modern learning architectures are over-parametrized and are trained to interpolate the data by driving the empirical loss (classification and regression) close to zero. While it is still unclear why these interpolated solutions perform well on test data, we show that these regimes allow for fast convergence of SGD, comparable in number of iterations to full gradient descent. For convex loss functions we obtain an exponential convergence bound for {\it mini-batch} SGD parallel to that for full gradient descent. We show that there is a critical batch size $m^*$ such that: (a) SGD iteration with mini-batch size $m\leq m^*$ is nearly equivalent to $m$ iterations of mini-batch size $1$ (\emph{linear scaling regime}). (b) SGD iteration with mini-batch $m> m^*$ is nearly equivalent to a full gradient descent iteration (\emph{saturation regime}). Moreover, for the quadratic loss, we derive explicit expressions for the optimal mini-batch and step size and explicitly characterize the two regimes above. The critical mini-batch size can be viewed as the limit for effective mini-batch parallelization. It is also nearly independent of the data size, implying $O(n)$ acceleration over GD per unit of computation. We give experimental evidence on real data which closely follows our theoretical analyses. Finally, we show how our results fit in the recent developments in training deep neural networks and discuss connections to adaptive rates for SGD and variance reduction.

==> related.tex <==
Sublinear convergence for non-strongly convex smooth loss~\cite{shalev2014understanding} (Section 14.5.2), linear convergence for strongly convex smooth loss~\cite{needell2014stochastic} (Theorem 2.1)~\cite{moulines2011non}.

\subsection{Ruslan's Deep Learning Tutorial (\href{https://simons.berkeley.edu/talks/ruslan-salakhutdinov-01-26-2017-1}{video}, \href{http://www.cs.cmu.edu/~rsalakhu/talk_Simons_part1_pdf.pdf}{slide})}

{\bf 23:32} "Optimization is much easier in an over-parametrized space." (for single layer neural network)

\noindent{\bf 30:35} Overfitting: high variance / low bias
(linear system: low variance / high bias, 
complex system: high variance / low bias)

\noindent{\bf 49:51} "The best way to solve the problem from practical stand of point is you build a very big system. If you remove any of these regularization like dropout or l2, basically you want to make sure you hit the zero training error. Because if you don't, you somehow waste the capacity of the model."

\noindent{\bf 50:33} "It seems like working/doing optimization in an over-paramatrized space is an easier task." (Misha here)



\subsection{Randomized Kaczmarz~\cite{kaczmarz1937angenaherte} (\href{http://www.cs.ubc.ca/~nickhar/W15/Lecture21Notes.pdf}{note})}

Consider linear system $A \bx = \bb$ where $A \defeq (\ba_1, \ldots, \ba_m)^T$, $\bb \defeq (b_1, \ldots, b_m)^T$, and $\ba_1, \dots, \ba_m, \bx \in \mathbb{R}^n$. If the system has unique solution $\bx^*$, Kaczmarz method approximates it through iteration,
$$
\bx_{t+1} \leftarrow \arg\min_{\bx | \ba_{i_{t}}^T \bx = b_{i_{t}}} \norm{\bx - \bx_t}^2
$$

By finding the stationary point of corresponding Lagrangian, the iteration is equivalent to
$$
\bx_{t+1} \leftarrow \bx_t -
\frac{\ba_{i_{t}}^T \bx - b_{i_{t}}}{\norm{\ba_{i_{t}}}^2} \ba_{i_{t}}
$$
which is essentially stochastic gradient decent with adaptive step size $\frac{1}{{\norm{\ba_{i_{t}}}^2}}$. The stochastic loss in this case is $\ell_{i_t} \defeq \frac{1}{2}(\ba_{i_t}^T \bx - b_{i_t})^2$.

When $i_t \sim [m]$, the method has exponential convergence rate,
$$
\expect{\norm{\bx_{t+1} - \bx^*}^2}
\leq (1 - \frac{\lambda_{min}(A)^2}{m \norm{A}_{\infty}^2})
\expect{\norm{\bx_{t} - \bx^*}^2}
$$
Note that the convergence of Kaczmarz method does not rely on the existence and uniqueness of $\bx^*$.

\subsection{Distributed SGD}
In a distributed environment comprised of $N$ machines, there are usually two ways to perform SGD, synchronous and asynchronous. 
In the synchronous setting, each machine keeps the same snapshot of the model, calculates update for different mini-batch. Then they form the final update by averaging all updates.
%At the beginning of one iteration, each machine will get an (independently sampled) mini-batch and calculates the update accordingly. Then updates from all machines will be combined (mostly through average). Before proceeding to the next iteration, the latest snapshot of the model.
It is essentially equivalent to adopting $N$ times larger mini-batch.

In the asynchronous setting, each machine may keep a different snapshot of the model and update from one machine may get overwritten by updates from the others. When updates from all machines are not overlapped, the asynchronous setting performs $N$ times more iterations in the same amount of time.
\cite{de2015taming} presents a convergence analysis on such a setting with an extra sparsity assumption. The assumption implies that an update from one machine rarely overlap with updates from other machines.

The industry initially shows more interests in the asynchronous setting since it is more scalable. Several systems have since been developed targeting this setting, e.g. Tensorflow~\cite{abadi2016tensorflow} (Google) and Mxnet~\cite{chen2015mxnet}. Popular system like Caffe~\cite{jia2014caffe} also has extensions to support such setting. Note that all these systems also support the synchronous setting by default.

However, as discussed in \cite{chen2016revisiting}, the asynchronous setting introduces more noise. When scaling up over a few dozens of machines, the noise hurts the training in the long run. Thus a shift of focus onto the synchronous setting seems ongoing.
A prominent example is the recent work~\cite{goyal2017accurate} by Facebook. An interesting trick adopted by this work is the linear scaling rule (for step size). When $N$ machines are used, this rule suggests to increase the step size by a factor of $N$, which likely contributes to the acceleration of SGD convergence. Similar scaling factors are also used in \cite{krizhevsky2014one}  ($\sqrt{N}$ in theory while $N$ in practice) and \cite{chen2016revisiting} ($N$). \cite{bottou2016optimization} (p. 30) gives some intuitive explanations on its effectiveness using the variance of the (mini-batch) stochastic gradient.

